Leveraging Content and Context Cues for Low-Light Image Enhancement

Low-light conditions have an adverse impact on machine cognition, limiting the performance of computer vision systems in real life. Since low-light data is limited and difficult to annotate, we focus on image processing to enhance low-light images and improve the performance of any downstream task model, instead of fine-tuning each of the models which can be prohibitively expensive. We propose to improve the existing zero-reference low-light enhancement by leveraging the CLIP model to capture image prior and for semantic guidance. Specifically, we propose a data augmentation strategy to learn an image prior via prompt learning, based on image sampling, to learn the image prior without any need for paired or unpaired normal-light data. Next, we propose a semantic guidance strategy that maximally takes advantage of existing low-light annotation by introducing both content and context cues about the image training patches. We experimentally show, in a qualitative study, that the proposed prior and semantic guidance help to improve the overall image contrast and hue, as well as improve background-foreground discrimination, resulting in reduced over-saturation and noise over-amplification, common in related zero-reference methods. As we target machine cognition, rather than rely on assuming the correlation between human perception and downstream task performance, we conduct and present an ablation study and comparison with related zero-reference methods in terms of task-based performance across many low-light datasets, including image classification, object and face detection, showing the effectiveness of our proposed method.

==> Sections/WorkingDraft.tex <==
\clearpage

!* delete 

\rebuttal{!*}

!* add a comment about that direct comparison is not possible



% \begin{table}[]
% \rebuttalcontainer
% \caption{\rebuttalcontainer Quantitative comparisons of the proposed and related paired and unpaired data methods in terms of the PSNR and SSIM metrics on the VE-LOL \cite{liu2021benchmarking} dataset. The computational complexity is calculated for processing a $1024 \times 1024$ px image.}
% \label{tab:cross-comparison-psnr}

% \centering
% \scriptsize

% \begin{tabular}{c|ccc}
% \hline

% Method & PSNR $\uparrow$ & SSIM $\uparrow$ 
% & \tiny{Complexity} \\ 
%  &  & & MACs $\downarrow$ \\ 
% \hline

% \rule{0pt}{2ex} (no enhancement) & 10.23 & 0.29 \\
% \hline

% \multicolumn{1}{l|}{PAIRED DATA METHODS:} & \\

% SNR+SKF \cite{Wu_2023_CVPR} \textsuperscript{(CVPR2023)} & 23.40 & 0.76 & 886G \\

% DRBN+SKF \cite{Wu_2023_CVPR} \textsuperscript{(CVPR2023)} & 21.02 & 0.76 & 560G \\

% PairLIE \cite{Fu_2023_CVPR_Learning} \textsuperscript{(CVPR2023)} & 18.38 & 0.69  & 359G \\

% Wavelet-based Diffusion \cite{jiang2023low} \textsuperscript{(SIGGRAPH ASIA 2023)} & 25.07 & 0.79 & 1410G \\

% \hline % \rule{0pt}{3ex}


% \multicolumn{1}{l|}{UNPAIRED DATA/UNSUPERVISED:} & \\

% CLIP-LIT \cite{liang2023iterative} \textsuperscript{(ICCV2023)} & 14.17 & 0.55 & 292G \\

% PIE {} {} \cite{liang2024pie} \textsuperscript{(IJCV2024)} & 13.46 & 0.52 & 83G \\

% QuadPrior (FP16) \cite{wang2024zero} \textsuperscript{(CVPR24)} & 17.24 & 0.72 & 13740G \\

% \hline % \rule{0pt}{2ex}

% Ours & 15.62 & 0.57 & 83G \\

% \hline
% \end{tabular}
% % \\ \aftertable
% \end{table}






















\clearpage










% \begin{figure*}[t]

%     \captionsetup[subfigure]{justification=centering}
%     \rebuttalcontainer 
%     \centering
%     \small

%     % DSC01544
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/000000_ORIG_DSC01544.JPG}
%         \caption*{}
% %         \caption*{Input }  
%     \end{subfigure} %
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/RUAS_DSC01544.JPG}
%         \caption*{}
% %         \caption*{RUAS \cite{liu2021retinex}}
%     \end{subfigure} %
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/SGLLIE_DSC01544.JPG}
%         \caption*{}
% %         \caption*{SGZ \cite{zheng2022semantic}}
%     \end{subfigure} %
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/240516_005131_CLIP_ZDCE_FULL_E_DSC01544.JPG}
%         \caption*{}
% %         \caption*{Zero-DCE \cite{guo2020zero}}
%     \end{subfigure} % content
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/SCI_DSC01544.JPG}
%         \caption*{}
% %         \caption*{SCI \cite{ma2022toward}}
%     \end{subfigure} %context
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/240516_181048_from_240507_1354_DSC01544.JPG}
%         \caption*{}
% %         \caption*{Ours}
%     \end{subfigure} %contentcontext

% \vspace{-1.2em}


% %     % DSC02093
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/000000_ORIG_DSC02093.JPG}
% %         \caption*{} 
% %     \end{subfigure} %
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/RUAS_DSC02093.JPG}
% %         \caption*{}
% %     \end{subfigure} %
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/SGLLIE_DSC02093.JPG}
% %         \caption*{}
% %     \end{subfigure} %
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/240516_005131_CLIP_ZDCE_FULL_E_DSC02093.JPG}
% %         \caption*{}
% %     \end{subfigure} % content
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/SCI_DSC02093.JPG}
% %         \caption*{}
% %     \end{subfigure} %context
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/240516_181048_from_240507_1354_DSC02093.JPG}
% %         \caption*{}
% %     \end{subfigure} %contentcontext

% % \vspace{-1.2em}


%     % DSC02620
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/000000_ORIG_DSC02620.JPG}
%         \caption*{}
% %         \caption*{Input }  
%     \end{subfigure} %
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/RUAS_DSC02620.JPG}
%         \caption*{}
% %         \caption*{RUAS \cite{liu2021retinex}}
%     \end{subfigure} %
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/SGLLIE_DSC02620.JPG}
%         \caption*{}
% %         \caption*{SGZ \cite{zheng2022semantic}}
%     \end{subfigure} %
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/240516_005131_CLIP_ZDCE_FULL_E_DSC02620.JPG}
%         \caption*{}
% %         \caption*{Zero-DCE \cite{guo2020zero}}
%     \end{subfigure} % content
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/SCI_DSC02620.JPG}
%         \caption*{}
% %         \caption*{SCI \cite{ma2022toward}}
%     \end{subfigure} %context
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/240516_181048_from_240507_1354_DSC02620.JPG}
%         \caption*{}
% %         \caption*{Ours}
%     \end{subfigure} %contentcontext

% \vspace{-1.2em}


%     % DSC03247
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/000000_ORIG_DSC03247.JPG}
%         \caption*{}
% %         \caption*{Input }  
%     \end{subfigure} %
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/RUAS_DSC03247.JPG}
%         \caption*{}
% %         \caption*{RUAS \cite{liu2021retinex}}
%     \end{subfigure} %
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/SGLLIE_DSC03247.JPG}
%         \caption*{}
% %         \caption*{SGZ \cite{zheng2022semantic}}
%     \end{subfigure} %
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/240516_005131_CLIP_ZDCE_FULL_E_DSC03247.JPG}
%         \caption*{}
% %         \caption*{Zero-DCE \cite{guo2020zero}}
%     \end{subfigure} % content
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/SCI_DSC03247.JPG}
%         \caption*{}
% %         \caption*{SCI \cite{ma2022toward}}
%     \end{subfigure} %context
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/240516_181048_from_240507_1354_DSC03247.JPG}
%         \caption*{}
% %         \caption*{Ours}
%     \end{subfigure} %contentcontext

% % \vspace{-1.2em}


% %     % DSC_3652
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/000000_ORIG_DSC_3652.JPG}
% %         \caption*{} 
% %     \end{subfigure} %
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/RUAS_DSC_3652.JPG}
% %         \caption*{}
% %     \end{subfigure} %
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/SGLLIE_DSC_3652.JPG}
% %         \caption*{}
% %     \end{subfigure} %
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/240516_005131_CLIP_ZDCE_FULL_E_DSC_3652.JPG}
% %         \caption*{}
% %     \end{subfigure} % content
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/SCI_DSC_3652.JPG}
% %         \caption*{}
% %     \end{subfigure} %context
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/240516_181048_from_240507_1354_DSC_3652.JPG}
% %         \caption*{}
% %     \end{subfigure} %contentcontext

% % \vspace{-1.2em}



% %     % 0822_DSC07109
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/000000_ORIG_0822_DSC07109.JPG}
% %         \caption*{} 
% %     \end{subfigure} %
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/RUAS_0822_DSC07109.JPG}
% %         \caption*{}
% %     \end{subfigure} %
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/SGLLIE_0822_DSC07109.JPG}
% %         \caption*{}
% %     \end{subfigure} %
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/240516_005131_CLIP_ZDCE_FULL_E_0822_DSC07109.JPG}
% %         \caption*{}
% %     \end{subfigure} % content
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/SCI_0822_DSC07109.JPG}
% %         \caption*{}
% %     \end{subfigure} %context
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/240516_181048_from_240507_1354_0822_DSC07109.JPG}
% %         \caption*{}
% %     \end{subfigure} %contentcontext

% % \vspace{-1.2em}


% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/CROP_000000_ORIG_LIME_5.png}
% %         \caption*{Input } 
% %     \end{subfigure} %
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/CROP_RUAS_LIME_5.png}
% %         \caption*{RUAS \cite{liu2021retinex}}
% %     \end{subfigure} %
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/CROP_SGLLIE_LIME_5.png}
% %         \caption*{SGZ \cite{zheng2022semantic}}
% %     \end{subfigure} %
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/CROP_240516_005131_CLIP_ZDCE_FULL_ENSEMBLE_batch8x224_json_OV_LIME_5.png}
% %         \caption*{Zero-DCE \cite{guo2020zero}}
% %     \end{subfigure} % content
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/CROP_SCI_LIME_5.png}
% %         \caption*{SCI \cite{ma2022toward}}
% %     \end{subfigure} %context
% %     \begin{subfigure}{.14\textwidth}
% %       \centering
% %         \includegraphics[width=1\linewidth]{Images/bboxes-figures/CROP_240516_181048_XXXbatch8x224_json_OV_CLIP_CONTENT_TRAINED_CONTEXT_TRAINED_PAUG_CPT_FROM_FT_DISCRIMINATOR_AND_AUG_LIME_5.png}
% %         \caption*{Ours}
% %     \end{subfigure} %contentcontext

% \vspace{-1.2em}

%     % DSC_3397
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/000000_ORIG_DSC_3397.JPG}
%         % \caption*{}
%         \caption*{Input }  
%     \end{subfigure} %
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/RUAS_DSC_3397.JPG}
%         % \caption*{}
%         \caption*{RUAS \cite{liu2021retinex}}
%     \end{subfigure} %
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/SGLLIE_DSC_3397.JPG}
%         % \caption*{}
%         \caption*{SGZ \cite{zheng2022semantic}}
%     \end{subfigure} %
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/240516_005131_CLIP_ZDCE_FULL_E_DSC_3397.JPG}
%         % \caption*{}
%         \caption*{Zero-DCE \cite{guo2020zero}}
%     \end{subfigure} % content
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/SCI_DSC_3397.JPG}
%         % \caption*{}
%         \caption*{SCI \cite{ma2022toward}}
%     \end{subfigure} %context
%     \begin{subfigure}{.14\textwidth}
%       \centering
%         \includegraphics[width=1\linewidth]{Images/bboxes-figures/240516_181048_from_240507_1354_DSC_3397.JPG}
%         % \caption*{}
%         \caption*{Ours} 
%     \end{subfigure} %contentcontext

% \yololegend
%     \caption{\rebuttalcontainer Qualitative results of object detection using Yolo-World model \cite{cheng2024yolo} on the NOD \cite{morawski2021nod}. Instead of assuming correlation between human and machine cognition, we propose to directly optimize the enhancement for machine cognition, leading to reduction in prediction noise. Moreover, our proposed image prior additionally helps to generalize to bright images, avoiding overexposure which may adversely impact downstream task models.  !*}
    



    
% %         \caption*{Input } 
% %         \caption*{RUAS \cite{liu2021retinex}}
% %         \caption*{SGZ \cite{zheng2022semantic}}
% %         \caption*{Zero-DCE \cite{guo2020zero}}
% %         \caption*{SCI \cite{ma2022toward}}
% %         \caption*{Ours}

%     \label{fig:comparisonbbox}
% \end{figure*}

==> Tables/Tab_IODom.tex <==
% &  &  & !* & !* & \firstbest{!*} & !* & !* \\

\begin{table*}[t]
    \caption{Task-based evaluation of the proposed method, in the in- and out-of-domain scenarios}
    \label{tab:ablation-iodom}
    
    \centering
    \footnotesize
    \begin{tabular}{cc|cccccc}
    \hline
    
      Method & In-domain & NOD \cite{morawski2021nod} & NOD SE \cite{morawski2021nod} &  LOD \cite{hong2021crafting} & ExDark \cite{loh2019getting} & ExDark \cite{loh2019getting} & DarkFace \cite{poor_visibility_benchmark} \\
    
     & & mAP $\uparrow$ & mAP $\uparrow$ & mAP $\uparrow$ & mAP $\uparrow$ & class. acc. $\uparrow$ & mAP@.5 $\uparrow$ \\ \hline
     
     baseline \cite{guo2020zero} & \checkmarkx & 41.2\% & 22.4\% & 40.9\% & 34.1\% & 43.7\% & 35.6\%  \\

     proposed method & \checkmarkx & 42.3\% & 25.4\% & 44.4\% & 36.9\% & 45.9\% & 37.3\% \\ \hline
        
    baseline \cite{guo2020zero} & \checkmark & 40.4\% & 22.0\% & 38.6\% & 33.3\% & 40.9\% & 33.8\%  \\

     proposed method & \checkmark & 43.9\%  & 27.0\%  & 47.1\%  & 39.9\%  & 42.5\%  & 42.1\% \\
    
    \hline
    \end{tabular}
    \end{table*}
    
    
